Adaptable Agent Populations via a Generative Model of Policies

In the natural world, life has found innumerable ways to survive and often thrive. Between and even within species, each individual is in some manner unique, and this diversity lends adaptability and robustness to life. In this work, we aim to learn a space of diverse and high-reward policies on any given environment. To this end, we introduce a generative model of policies, which maps a low-dimensional latent space to an agent policy space. Our method enables learning an entire population of agent policies, without requiring the use of separate policy parameters. Just as real world populations can adapt and evolve via natural selection, our method is able to adapt to changes in our environment solely by selecting for policies in latent space. We test our generative model's capabilities in a variety of environments, including an open-ended grid-world and a two-player soccer environment. Code, visualizations, and additional experiments can be found at https://kennyderek.github.io/adap/.

==> biblio.tex <==
%% This defines the bibliography file (main.bib) and the bibliography style.
%% If you want to create a bibliography file by hand, change the contents of
%% this file to a `thebibliography' environment.  For more information 
%% see section 4.3 of the LaTeX manual.
% \begin{singlespace}
% \bibliographystyle{plainnat}
\bibliography{main}
% \end{singlespace}




==> unused.tex <==
% \section{Robustness-Performance Tradeoff}

% We want to understand the relationship between policy space diversity on general adaptation performance, and highest-quality performance. We let general adaptation performance be the score of the G against \texttt{\{updown0, updown1, straight, stand, and random\}}, as these are naive and exploitable opponents that may not be encountered in the standard self-play curriculum. We measure highest-quality-performance as the score of G against our hard-coded bot, which as seen in the above figure, is a strong opponent against all methods.

% In our experiment, we use the Div + Mult model and vary only the diversity regularizer coefficient. All other parameters remain the same as in the prior experiment. We use coefficient settings {0.0, 0.1, 0.2, 0.3, 0.4}. Note that setting 0.0 is equivalent to Vanilla PPO with entropy regularization. We then test each method against our suite of hand-coded bots.

% \begin{figure}[h]
% \includegraphics[width=1\linewidth]{app_figures/RobustnessPerformanceTradeoffNew.png}
% \centering
% \caption{Robustness and Performance as a Function of Capacity and Diversity Regularizer Coefficient}
% \label{robustnessVsperf}
% \end{figure}

% As seen in the Figure \ref{robustnessVsperf}, there is a strong positive relationship between higher diversity regularizer coefficient, and score against the \texttt{\{updown0, updown1, straight, stand, and random\}} tasks. On the other hand, as the diversity regularizer coefficient increases, performance against our hand-coded bot remains constant. Additionally, modulating network capacity is not a major factor in being able to fit large number of policies into the weights $\theta$ of $G_{\theta}$. We conclude that, in general, it is not necessary to sacrifice adaptability for performance against a single task. For example, if there exists a worse-case-optimal policy in an environment, there is no reason it would be excluded from the learned policy space.


% \section{How Model Architecture and Context Distribution affects Multi-Modality}

% We train a policy $\pi$ to maximize 1-step expected rewards given observation of the domain $x \in [0, 1]$ and target $f(x) \in [0, 1]$. The output of $\pi$ is $\mu$ and $\sigma^2$, from which we generate action $a \sim \mathcal{N}(\mu, \sigma^2)$. We use the REINFORCE algorithm, and compute advantage by normalizing the reward across a batch of samples $(s, a, r)$, where $s$ is the $(x, z)$ input pair and $a$ = the $y$ prediction. Crucially, we normalize rewards with across a batch collected using the same latent $z$, which essentially treats each latent vector as a unique `bucket,' similarly to how MapElites (\cite{mapelites}) only measures competition with individuals that are in the same bucket. Doing so is important, since otherwise we would hinder specialization and diversity by measuring the reward of a hypothetical latent vector $z_i$ that is currently attempting to diversify, against the reward of a currently high-performing hypothetical latent vector $z_j$. This would penalize $z_i$'s actions, when in reality, we want to encourage the diversification. In later experiments, we discard this sort of reward normalization in favor of using an actual value function that is able to account for these expected reward differences, conditional on the particular latent $z$.

% Reward is calculated as 
% $$\min_{f \in \mathcal{F}} \ -(a - f(x))^2$$
% where $\mathcal{F}$ is a family of functions in the multi-function environment. We use $$\mathcal{F} = \{
% f_1(x), f_2(x),f_3(x)\}$$
% where
% \begin{align*}
%   f_1(x) &= x^2 + 0.5\\
%   f_1(x) &= -x\\
%   f_3(x) &= x - 0.75
% \end{align*}
% % $$f_1(x) = x^2 + 0.5$$
% % $$f_1(x) = -x$$
% % $$f_3(x) = x - 0.75\}$$

% In this experiment we explore the influence of model architecture, and latent distribution, and use of our diversity regularizer on the multi-modality of the policy generator.

% \textit{Model Architectures}
% \begin{itemize}
%     \item Concatenation Model. A latent context is concatenated to the flattened environmental observation.
%     \item Multiplicative Model. The latent context is multiplicatively integrated with a learned embeddings of the environmental observation.
% \end{itemize}

% \textit{Context Distributions of size $3$}
% \begin{itemize}
%     \item Uniform $3$-Categorical ($k$-dim one-hot)
%     \item $\mathbb{R}^3 \sim $ Unif[0, 1]
%     \item $\mathbb{R}^3 \sim $ Unit Sphere, centered at 0, 0. Thus the magnitude of the latent vector $|z| = 1$.
% \end{itemize}

% \paragraph{Results}
% \begin{figure}[h]
% \begin{center}
% \includegraphics[width=1\linewidth]{app_figures/functionWorld.png}
% \end{center}
% \label{funcs}
% \caption{Using a Multi-Modal Policy to Model Three Different Functions}
% \small Target functions are shown in dotted lines. Policy predictions are shown in solid colored lines, where each $(x, y)$ point is visualized in the RGB color directly proportional to it's latent vector. Importantly, we observe that using a concatenation model does not provide the generator enough representational flexibility to fit to all three functions in $\mathcal{F}$.
% \end{figure}

% As seen in \ref{funcs}, both model architecture and latent distribution are important in learning a multi-modal policy space.

% The first thing to note is that using our multiplicative model, a type of Stochastic Neural Network, has a significant impact on the ability of our generator to learn a multi-modal space of policies. Simply using the concatenation model does not provide the generator enough representational flexibility to fit to all three functions in $\mathcal{F}$.

% Our second observation is that using continuous latent vectors hinders how well any one latent can fit to a particular function. However, we believe using continuous latent space still provides major benefits over a discrete latent space. First and foremost, a discrete latent space will only be able to find a limited set of distinct agent policies. On the other hand, a continuous latent space of policies offers the enticing possibility of finding as many policies as the generator $G$ can fit. Additionally, a continuous latent space offers the ability to interpolation and optimization policies in the latent space.

% In all following experiments, unless otherwise specified, we use continuous contexts sampled from the 3-dimensional unit sphere.

